Preparing for Kyber in Securing Intelligent Transportation Systems Communications: A Case Study on Fault-Enabled Chosen-Ciphertext Attack

Intelligent transportation systems (ITS) are characterized by wired or wireless communication among different entities, such as vehicles, roadside infrastructure, and traffic management infrastructure. These communications demand different levels of security, depending on how sensitive the data is. The national ITS reference architecture (ARC-IT) defines three security levels, i.e., high, moderate, and low-security levels, based on the different security requirements of ITS applications. In this study, we present a generalized approach to secure ITS communications using a standardized key encapsulation mechanism, known as Kyber, designed for post-quantum cryptography (PQC). We modified the encryption and decryption systems for ITS communications while mapping the security levels of ITS applications to the three versions of Kyber, i.e., Kyber-512, Kyber-768, and Kyber-1024. Then, we conducted a case study using a benchmark fault-enabled chosen-ciphertext attack to evaluate the security provided by the different Kyber versions. The encryption and decryption times observed for different Kyber security levels and the total number of iterations required to recover the secret key using the chosen-ciphertext attack are presented. Our analyses show that higher security levels increase the time required for a successful attack, with Kyber-512 being breached in 183 seconds, Kyber-768 in 337 seconds, and Kyber-1024 in 615 seconds. In addition, attack time instabilities are observed for Kyber-512, 768, and 1024 under 5,000, 6,000, and 8,000 inequalities, respectively. The relationships among the different Kyber versions, and the respective attack requirements and performances underscore the ITS communication security Kyber could provide in the PQC era.

==> 07_Declarations_title_page.tex <==
\section*{Declarations }
\subsection*{Competing Interests}
The authors have no conflicts of interest to declare relevant to this article's content.
\subsection*{Authors' Contributions}
The authors confirm their contribution to the paper as follows: study conception and design: K. Zhang, M.S. Salek, A. Wang, M. Chowdhury, Y. Lao; analysis and interpretation of results: K. Zhang, M.S. Salek, A. Wang, Y. Lao; draft manuscript preparation: K. Zhang, M.S. Salek, A. Wang, M. Chowdhury, Y. Lao, M. Rahman. All authors reviewed the results and approved the final version of the manuscript.
